Resistance Scaling on $4N$-Carpets

The $4N$ carpets are a class of infinitely ramified self-similar fractals with a large group of symmetries. For a $4N$-carpet $F$, let $\{F_n\}_{n \geq 0}$ be the natural decreasing sequence of compact pre-fractal approximations with $\cap_nF_n=F$. On each $F_n$, let $\mathcal{E}(u, v) = \int_{F_N} \nabla u \cdot \nabla v \, dx$ be the classical Dirichlet form and $u_n$ be the unique harmonic function on $F_n$ satisfying a mixed boundary value problem corresponding to assigning a constant potential between two specific subsets of the boundary. Using a method introduced by Barlow and Bass (1990), we prove a resistance estimate of the following form: there is $\rho=\rho(N) > 1$ such that $\mathcal{E}(u_n, u_n)\rho^{n}$ is bounded above and below by positive constants independent of $n$. Such estimates have implications for the existence and scaling properties of Dirichlet forms on $F$.

==> dodec0.tex <==
\draw (0.8365163, 0.4829629)--(0.0, 0.0);
\draw (-0.4829629, 0.8365163)--(0.0, 0.0);
\draw (-1.6653345e-16, -0.9659258)--(0.0, 0.0);


==> dodecaF0.tex <==
\draw (0.8365163, 0.4829629)--(0.0, 0.0);
\draw (-0.4829629, 0.8365163)--(0.0, 0.0);
\draw (-1.6653345e-16, -0.9659258)--(0.0, 0.0);


==> octa0.tex <==
\draw (0.6532815, 0.6532815)--(0.0, 0.0);
\draw (-0.6532815, 0.6532815)--(0.0, 0.0);
\draw (-1.6653345e-16, -0.9238795)--(0.0, 0.0);


==> octaF0.tex <==
None] (0.6532815, 0.6532815)--(0.0, 0.0);
None] (-0.6532815, 0.6532815)--(0.0, 0.0);
None] (-1.6653345e-16, -0.9238795)--(0.0, 0.0);

